ESPnet-SLU: Advancing Spoken Language Understanding through ESPnet

As Automatic Speech Processing (ASR) systems are getting better, there is an increasing interest of using the ASR output to do downstream Natural Language Processing (NLP) tasks. However, there are few open source toolkits that can be used to generate reproducible results on different Spoken Language Understanding (SLU) benchmarks. Hence, there is a need to build an open source standard that can be used to have a faster start into SLU research. We present ESPnet-SLU, which is designed for quick development of spoken language understanding in a single framework. ESPnet-SLU is a project inside end-to-end speech processing toolkit, ESPnet, which is a widely used open-source standard for various speech processing tasks like ASR, Text to Speech (TTS) and Speech Translation (ST). We enhance the toolkit to provide implementations for various SLU benchmarks that enable researchers to seamlessly mix-and-match different ASR and NLU models. We also provide pretrained models with intensively tuned hyper-parameters that can match or even outperform the current state-of-the-art performances. The toolkit is publicly available at https://github.com/espnet/espnet.

==> sections/related.tex <==
\section{Related Work}

Related Work goes here. 

==> tables/compare_pretrain_ASR.tex <==
\begin{table}[]
\begin{tabular}{l|c}
Pretrain Model                                                             & SLU  \\\toprule
Hubert                         & 83.3 \\
TERA    & 83.4 \\
Wav2vec2  & N/A \\
VQ-APC & N/A \\
\bottomrule
\end{tabular}
\caption{The table records
the impact of pretrained ASR models on Intent Classification accuracy
on the SLURP Dataset \cite{SLURP} .
}
\label{tbl:compare_pretrain}
\end{table}

==> tables/espnet_comparison_decoder.tex <==
\begin{table}[!hbp]
\caption{Comparison of available decoders with other open-source End to End Spoken Language Understanding toolkits in January 2022
}
\label{tbl:espnet_comp}
\centering
 \resizebox {\linewidth} {!} {
\begin{tabular}{l|ccccc}
\toprule
 & Alexa\cite{agrawal2020tie} & Lugosch\cite{Lugosch_FSC} & CoraJung \cite{cha2021speak} & SpeechBrain\cite{SpeechBrain} &  \bf{ESPnet-SLU} \\\midrule
Classifier & \checkmark &  & & \checkmark & \\
RNN &  & \checkmark & \checkmark & \checkmark & \checkmark \\
Transformer & & & & \checkmark  & \checkmark \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/result_DEMO.tex <==
\begin{table}[]
\begin{tabular}{l|cc}
  & Noisy Speech & Mixed Speech   \\\toprule
SLU & 73.1   &  \\
SE+ SLU & 81.4 & \\
SS+ SLU & & \\
\bottomrule
\end{tabular}
\caption{The table records
the Intent Classification accuracy
on the Fluent Speech Commands Dataset \cite{Lugosch_FSC} for noisy and mixed speech.
}
\label{tbl:Demo}
\end{table}

